Evaluating the Tradeoff Between Abstractiveness and Factuality in Abstractive Summarization

Neural models for abstractive summarization tend to generate output that is fluent and well-formed but lacks semantic faithfulness, or factuality, with respect to the input documents. In this paper, we analyze the tradeoff between abstractiveness and factuality of generated summaries across multiple datasets and models, using extensive human evaluations of factuality. In our analysis, we visualize the rates of change in factuality as we gradually increase abstractiveness using a decoding constraint, and we observe that, while increased abstractiveness generally leads to a drop in factuality, the rate of factuality decay depends on factors such as the data that the system was trained on. We introduce two datasets with human factuality judgements; one containing 10.2k generated summaries with systematically varied degrees of abstractiveness; the other containing 4.2k summaries from five different summarization models. We propose new factuality metrics that adjust for the degree of abstractiveness, and we use them to compare the abstractiveness-adjusted factuality of previous summarization works, providing baselines for future work.

==> automatic_metric.tex <==
To automatically measure the factual consistency of summaries with respect to their inputs, we use two entailment-based metrics: DAE \cite{goyal-durrett-2020-evaluating,goyal-durrett-2021-annotating} and FactCC \cite{kryscinski2020evaluating} and two metrics based on question answering: FEQA \cite{durmus2020feqa} and QAGS \cite{wang2020asking}.
\textbf{DAE} is an entailment model that classifies the factuality of the dependency arcs in the summary, resulting in fine-grained judgements at the subsentence level.
\textbf{FactCC} is a BERT-based binary classifier trained on sentence pairs derived from rules. We apply FactCC separately to each summary sentence and use the mean score per summary; when applying FactCC to a sentence we shorten the input document by selecting the ten sentences with the highest cosine embedding similarity \cite{conneau-etal-2017-supervised}. 
We also fine-tune the provided FactCC model further on the ANLI dataset \cite{nie2020adversarial}; we call this variant \textbf{FactCC$_A$}.
\textbf{FEQA} generates questions from masked summary sentences whose masked entities are used as ``gold'' answers; these are compared to the answers obtained from a QA model on the input.
In \textbf{QAGS}, a question generation model generates questions from the summary, a QA model answers these questions from both summary and input, and the similarity of the answer pairs is evaluated.






==> feqa_abstractiveness.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{6pt}
\centering
\ra{0.9}
\begin{tabular}{@{}lrrrrrrrrr@{}}\toprule
 & \hspace{6mm} \multirow{2}{*}{$\lambda$}  & \multicolumn{3}{c}{Extraction} & \multicolumn{2}{c}{Perfect fusion} & \multicolumn{3}{c}{Novel $n$-grams} \\
& & Sentence & Span & Word & $k=2$ &
  $k\geq2$ & $n=1$ & $n=2$ & $n=3$  \\
\midrule	
CNN/DM & $1/\lambda_2$ & 29.93 & 5.82 & 36.88 & 16.47 & 21.51 & 0.62 & 5.94 & 11.61 \\
	& none & 15.4 & 5.12 & 38.1 & 20.18 & 28.16 & 1.51 & 11.39 & 21.53 \\
	& $\lambda_4$ & 0.51 & 0.52 & 18.44 & 26.12 & 44.9 & 4.3 & 30.56 & 53.57 \\
	& $\lambda_2$ & 0.03 & 0.05 & 4.7 & 12.67 & 30.47 & 10.06 & 52.65 & 80.07 \\
\addlinespace[1mm]
MN-500 & $1/\lambda_2$ & 9.95 & 9.81 & 11.69 & 10.8 & 15.24 & 11.32 & 27.83 & 38.72 \\
	& none & 4.86 & 4.72 & 6.7 & 7.72 & 11.3 & 16.92 & 39.5 & 53.27 \\
	& $\lambda_4$ & 0.57 & 0.72 & 2.28 & 4.56 & 7.84 & 22.74 & 53.86 & 71.46 \\
	& $\lambda_2$ & 0.04 & 0.26 & 0.64 & 1.74 & 3.01 & 32.79 & 71.54 & 88.29 \\
\addlinespace[1mm]
MN-800 & $1/\lambda_2$ & 13.33 & 14.01 & 13.65 & 11.87 & 17.34 & 7.06 & 20.27 & 30.73 \\
	& none & 7.23 & 7.94 & 9.24 & 9.99 & 15.2 & 11.16 & 30.29 & 44.04 \\
	& $\lambda_4$ & 0.76 & 1.11 & 2.83 & 6.17 & 11.57 & 16.6 & 46.54 & 65.94 \\
	& $\lambda_2$ & 0.08 & 0.28 & 0.72 & 2.45 & 4.59 & 25.73 & 65.87 & 85.75 \\
\addlinespace[1mm]
XSUM & $1/\lambda_1$ & 1.99 & 1.58 & 1.31 & 2.03 & 14.47 & 12.53 & 46.41 & 54.93 \\
	& $1/\lambda_2$ & 0.49 & 0.09 & 0.36 & 0.6 & 4.56 & 22.27 & 62.71 & 57.98 \\
	& none & 0.16 & 0.03 & 0.22 & 0.24 & 2.43 & 26.12 & 66.94 & 54.36 \\
	& $\lambda_4$ & 0.03 & 0.0 & 0.05 & 0.08 & 1.64 & 27.71 & 69.4 & 51.65 \\
	& $\lambda_2$ & 0.0 & 0.0 & 0.0 & 0.03 & 0.68 & 31.5 & 72.46 & 38.73 \\
\bottomrule
\end{tabular}
\caption{Abstractiveness metrics in FEQA \cite{durmus2020feqa} for the data points shown in
  \xfigref{trends}. $\lambda$ values denote decoding
  constraints (\secref{slider})}. \label{tab:decodings_feqa_abs}
\end{table*}

The abstractiveness metrics of a generated summary proposed in FEQA \cite{durmus2020feqa} fall into three categories: extraction, perfect fusion, and novel $n$-grams. The extraction measurements evaluate the ratio of summary sentences copied from sentences, sentence spans, and a subset of tokens in input document(s). The perfect fusion measurements the ratio of summary sentences copied from multiple sentences from input document(s). The novel $n$-grams measurements the ratio of tokens in a summary that do not present in input document(s). The metrics are presented in \tabref{decodings_feqa_abs}. We observe that most of the metrics reflect increasing abstractiveness with larger penalty for extractive fragments for different datasets, except for word extraction and perfect fusion on CNN/DM dataset, and novel trigrams on XSum dataset.

